Navigating Central Path with Electrical Flows: from Flows to Matchings, and Back

We present an $\tilde{O}(m^{10/7})=\tilde{O}(m^{1.43})$-time algorithm for the maximum s-t flow and the minimum s-t cut problems in directed graphs with unit capacities. This is the first improvement over the sparse-graph case of the long-standing $O(m \min(\sqrt{m},n^{2/3}))$ time bound due to Even and Tarjan [EvenT75]. By well-known reductions, this also establishes an $\tilde{O}(m^{10/7})$-time algorithm for the maximum-cardinality bipartite matching problem. That, in turn, gives an improvement over the celebrated celebrated $O(m \sqrt{n})$ time bound of Hopcroft and Karp [HK73] whenever the input graph is sufficiently sparse.

==> files/interior_point_proof.tex <==

\section{Proof of Theorem \ref{thm:main_interior_point}}\label{app:proof_main_interior_point}


We obtain the desired solution $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ out of the solution $(\ff^{t},\ss^{t},\vnu^{t})$ in two steps. The first one -- the descent step -- focuses on using the electrical flow $\hff^t$ associated to solution $(\ff^{t},\ss^{t},\vnu^{t})$ and the corresponding vertex potentials $\hphi^t$ to obtain a new, intermediate, solution $(\off^t,\oss^t,\ovnu^t)$. This intermediate solution is $\vsigma$-feasible and has $\hmu(\off^t,\oss^t,\ovnu^t)\leq (1-\delta^t)\hmu(\ff^{t},\ss^{t},\vnu^{t})$ as desired, but it might be not $\hgamma$-centered. To fix that, in the second -- centering -- step, we obtain the desired solution $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ out of $(\off^t,\oss^t,\ovnu^t)$. We describe and analyze both of these steps below. Note that each of these two steps requires only one computation of electrical flow and can be easily implemented to run in $\tO{\hm}$ time, as needed.

\paragraph{Descent Step}

Let $\hff^t$ be the electrical $\vsigma$-flow associated with the solution $(\ff^{t},\ss^{t},\vnu^{t})$ and let $\hvphi^t$ be the vertex potentials that induce $\hff^t$. Consider a new primal-dual solution $(\off^t,\oss^t,\ovnu^t)$ given by
\begin{eqnarray}
\of_e^t & := & (1-\delta^t) f_e^t + \delta^t \hf_e^t\\
\os_e^t & := & s_e^t - \frac{\delta^t}{(1-\delta^t)} (\hphi^t_u-\hphi^t_v)=s_e^t - \delta^t \frac{s_e^t}{(1-\delta^t)f_e^t} \hf_e^t\\
\onu_e^t& := & \nu^t_e,
\end{eqnarray}
for each arc $e=(v,u)$ in $\hG$, where $\delta^t$ satisfies conditions of the theorem and we used the definition \eqref{eq:hf_resistances} of the resistances that determine $\hff^t$, as well as, the relationship \eqref{eq:potential_flow_def} between electrical flow and the vertex potentials that induce it. 


Let us first note that as $\off^t$ is a convex combination of two $\vsigma$-flows -- the flows $\ff^t$ and $\hff^t$ -- it also is an $\hvsigma$-flow. Furthermore, as all $\nu_e^t\geq 1$, we have $\norm{\vrho(\hff^t,\ff^t)}{\vnu^t,4}\leq \inorm{\vrho(\hff^t,\ff^t)}$ and thus can conclude that for each arc $e$,
\begin{equation}
\label{eq:interior_bound_2}
\of_e^t  =  (1-\delta^t) f_e^t + \delta^t \hf_e^t \geq (1-\delta^t) f_e^t - \delta^t |\hf_e^t| =  (1-\delta^t - \delta^t \rho(\hff^t,\ff^t)_e) f_e^t \geq (1-\frac{1}{2}-\sqrt{\hgamma})f_e^t>0,
\end{equation}
and similarly
\[
\os_e^t = s_e^t - \delta^t \frac{s_e^t}{(1-\delta^t)f_e^t} \hf_e^t \geq s_e^t - \delta^t \frac{s_e^t}{(1-\delta^t)f_e^t} |\hf_e^t| = s_e^t - \delta^t \frac{s_e^t}{(1-\delta^t)f_e^t} \rho(\hff^t,\ff^t)_e \geq (1-\frac{\sqrt{\hgamma}}{2})s_e^t>0.
\]
So, $(\off^t,\oss^t,\ovnu^t)$ is $\vsigma$-feasible, as desired.

Let us now analyze the value of $\hmu(\off^t,\oss^t,\ovnu^t)$. To this end, observe that, for any arc $e$,
\begin{eqnarray}
\ohmu_e^t =\frac{\of^t_e \os_e^t}{\onu^t_e} & = & (\nu_e^t)^{-1}((1-\delta^t) f_e^t + \delta^t \hf_e^t)(s_e^t - \delta^t \frac{s_e^t}{(1-\delta^t)f_e^t} \hf_e^t)\notag\\
&=& (\nu_e^t)^{-1}\left((1-\delta^t)f_e^ts_e^t +  \delta^t \hf_e^t s_e^t - \delta^t \frac{s_e^t}{(1-\delta^t)f_e^t} \hf_e^t (1-\delta^t) f_e^t - (\delta^t)^2 \frac{s_e^t}{(1-\delta^t)f_e^t}(\hf_e^t)^2\right) \notag\\
&=& (\nu_e^t)^{-1}\left((1-\delta^t) \mu_e^t + \delta^t \hf_e^t s_e^t - \delta^t \hf_e^t s_e^t - (\delta^t)^2 \frac{s_e^t}{(1-\delta^t)} f_e^t \rho(\hff^t,\ff^t)_e^2\right)\label{eq:duality_change}\\
&=& \left(1-\delta^t- \frac{(\delta^t\rho(\hff^t,\ff^t)_e)^2}{(1-\delta^t)}\right) \hmu_e^t.\notag
\end{eqnarray}
So, by definition \eqref{eq:def_hmu} and the fact that $\frac{(\delta^t\rho(\hff^t,\ff^t)_e)^2}{(1-\delta^t)}\geq 0$ for all $e$, we see that 
\[
\hmu(\off^t,\oss^t,\ovnu^t)\leq (1-\delta^t) \hmu(\ff^{t},\ss^{t},\vnu^{t})
\]
and this inequality would be an equality if the second-order terms (i.e., terms quadratic in $\delta^t$) were ignored. (Also, if these terms were not present, the centrality of the solution would be preserved too.)

Finally, let us focus on analyzing the centrality of $(\off^t,\oss^t,\ovnu^t)$ and note that by definition \eqref{eq:def_centrality} and by \eqref{eq:duality_change} above we have
\begin{eqnarray}
\norm{\ohvmu^t-\hmu(\off^t,\oss^t,\ovnu^t)\onev}{\ovnu^t,2}^2 & \leq & \norm{\ohvmu^t-(1-\delta^t)\hmu(\ff^t,\ss^t,\vnu^t)\onev}{\ovnu^t,2}^2 \leq \sum_e \onu_e^t (\ohmu_e^t-(1-\delta^t)\hmu(\ff^t,\ss^t,\vnu^t))^2\notag\\
&=& \sum_e \nu_e^t \left( (1-\delta^t)(\hmu_e^t-\hmu(\ff^t,\ss^t,\vnu^t))-\frac{(\delta^t\rho(\hff^t,\ff^t)_e)^2}{(1-\delta^t)}\hmu^t_e\right)^2\notag\\
&\leq & 2 \left((1-\delta^t)^2\sum_e \nu_e^t (\hmu^t_e-\hmu(\ff^t,\ss^t,\vnu^t))^2 + \sum_e \nu_e^t \frac{(\delta^t\rho(\hff^t,\ff^t)_e)^4}{(1-\delta^t)^2}(\hmu_e^t)^2 \right)\label{eq:centrality_increase}\\
&\leq & 2 \left((1-\delta^t)^2\norm{\hvmu^t-\hmu(\ff^t,\ss^t,\vnu^t)\onev}{\vnu^t,2}^2 + \frac{(1+\hgamma)^2\hmu(\ff^t,\ss^t,\vnu^t)^2}{(1-\delta^t)^2} (\delta^t)^4  \sum_e \nu_e^t \rho(\hff^t,\ff^t)_e^4 \right)\notag\\
&\leq & 2 \left((1-\delta^t)^2 \hgamma^2 \hmu(\ff^t,\ss^t,\vnu^t)^2 + \frac{(1+\hgamma)^2\hmu(\ff^t,\ss^t,\vnu^t)^2}{(1-\delta^t)^2} (\delta^t)^4 \sum_e \nu_e^t \rho(\hff^t,\ff^t)_e^4 \right)\notag\\
&\leq & 2 \left((1-\delta^t)^2 \hgamma^2 + \frac{(1+\hgamma)^2}{(1-\delta^t)^2} (\delta^t)^4 \norm{\vrho(\hff^t,\ff^t)}{\vnu^t,4}^4 \right)\hmu(\ff^t,\ss^t,\vnu^t)^2\notag\\
&\leq& 9 \hgamma^2\hmu(\off^t,\oss^t,\ovnu^t)^2. \notag
\end{eqnarray}
In the above derivation, the first inequality follows as the $\norm{\vmu-t\onev}{\vnu,2}$ is always minimized by taking $t=\hmu(\ff,\ss,\vnu)$. We also used the fact that $(\ff^t,\ss^t,\vnu^t)$ is $\hgamma$-centered, Fact \ref{fa:central_vs_max_min} and the upperbound on $\delta^t$.

Therefore, we see that as a price of making progress on the duality gap, the centrality of our solution could deteriorate by a factor of at most three. 

\paragraph{Centering Step}

To alleviate this possible increase of the centrality, we apply a second step that restores the centrality back within the desired bounds while not increasing the duality gap (so to not to counter the progress on the duality gap that we just achieved).

To this end, consider a flow $\off^*$ in $\hG$ defined as
\begin{equation}
\label{eq:def_of_offstar}
\of^*_e := \frac{\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t}\of^t_e,
\end{equation}
for every arc $e$ of $\hG$. Note that the flow $\off^*$ might (and actually will) not be feasible in $\hG$, as some of $\of^*_e$ can be negative.

Now, consider a flow $\off'$ given by
\begin{equation}
\label{eq:offprime_def}
\of_e' := \of^t_e - \of^*_e = (1-\frac{\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t})\of^t_e=\frac{\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t}\of^t_e,
\end{equation}
for each arc $e$. Observe that $\off'$ is feasible in $\hG$ (i.e., $\of_e'\geq 0$, for all $e$) and 
\begin{equation}
\label{eq:perfect_centering_of_intermediate}
\frac{\of_e'\os_e^t}{\onu_e^t} = \frac{\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t\onu_e^t}\of^t_e \os_e^t = \hmu(\off^t,\oss^t,\ovnu^t),
\end{equation}
for each arc $e$. That is, $(\off',\oss^t,\ovnu^t)$ is $0$-centered with $\hmu(\off',\oss^t,\ovnu^t)=\hmu(\off^t,\oss^t,\ovnu^t)$.

So, this solution would be a perfect candidate for $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ except that the flow $\off'$ does not need to be a $\vsigma$-flow and thus this solution might not be $\vsigma$-feasible. 

To fix that -- and obtain our desired solution $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ -- let $\tvsigma$ be the demand vector of the flow $\off^*$, and consider an electrical $\tvsigma$-flow $\tff^t$ that corresponds to resistances
\begin{equation}
\label{eq:tfft_resistances}
\tr_e^t := \frac{\os_e^t}{\of'_e},
\end{equation}
for each arc $e$ and let $\tvphi$ be the corresponding vertex potentials.

Let us define $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ to be
\begin{eqnarray}
f_e^{t+1} & := & \of'_e + \tf_e^t\notag\\
s_e^{t+1} & := & \os_e^t - (\tphi^t_u-\tphi^t_v) =\os_e^t - \frac{\os_e^t}{\of_e'} \tf_e^t\label{eq:new_ff_t1_def}\\
\nu_e^{t+1}& := & \onu^t_e,\notag
\end{eqnarray}
for each arc $e=(v,u)$. 



Clearly, now $\ff^{t+1}$ is a $\vsigma$-flow, as desired. Let us analyze its centrality. To this end, let us fix some arc $e$, and notice that
\begin{eqnarray*}
\hmu^{t+1}_e &=& \frac{f_e^{t+1}s_e^{t+1}}{\nu_e^{t+1}}=\frac{(\of'_e + \tf_e^t)(\os_e^t - \frac{\os_e^t}{\of_e'}\tf_e^t)}{\nu_e^{t+1}}\\ &=&(\onu_e^{t})^{-1}\left(\of'_e\os_e^t+\os_e^t\tf_e^t-\os_e^t\tf_e^t-\frac{\os_e^t}{\of_e'} (\tf_e^t)^2\right)\\
&=&\hmu(\off^t,\oss^t,\ovnu^t)-\frac{\os_e^t}{\onu^t\of_e'} (\tf_e^t)^2,
\end{eqnarray*}
where we used \eqref{eq:perfect_centering_of_intermediate}. So, we see in particular that 
\[
\hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1})\leq \hmu(\off^t,\oss^t,\ovnu^t)\leq (1-\delta^t)\hmu(\ff^{t},\ss^{t},\vnu^{t}),
\]
as needed. 

Now, by our derivation above, we have that
\[
\norm{\hvmu^{t+1}-\hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1})\onev}{\vnu^{t+1},2}^2\leq \norm{\hvmu^{t+1}-\hmu(\off^{t},\ss^{t},\ovnu^{t})\onev}{\vnu^{t+1},2}^2 = \sum_e \onu_e^t \left(\frac{\os_e^t}{\onu^t_e\of_e'} (\tf_e^t)^2\right)^2.
\]

To bound the resulting expression, let us note that by Cauchy-Schwarz inequality and the fact that measures are always at least $1$ we have 
\[
\sum_e \onu_e^t \left(\frac{\os_e^t}{\onu^t_e\of_e'} (\tf_e^t)^2\right)^2\leq \left(\max_{e} \frac{\os_e^t}{\onu^t_e\of_e'} (\tf_e^t)^2\right)\left(\sum_{e} \frac{\os_e^t}{\of_e'} (\tf_e^t)^2\right)\leq \left(\sum_{e} \frac{\os_e^t}{\of_e'} (\tf_e^t)^2\right)^2.
\]

Now, the key insight here is that by \eqref{eq:tfft_resistances}, 
\[
\left(\sum_{e} \frac{\os_e^t}{\of_e'} (\tf_e^t)^2\right)^2=\left(\energy{\trr^t}{\tff^t}\right)^2.
\]
So, by bounding the energy of the electrical flow $\tf_e^t$ we will be able to bound the centrality of our solution $\hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$. 
To bound this energy, we will first bound the energy $\energy{\trr^t}{\off^*}$ of the flow $\off^*$ and use the fact that both $\off^*$ and $\tff^t$ are $\tvsigma$-flows and thus, by definition, $\tff^t$ is minimizing the energy among all the $\tvsigma$-flows. 

Observe that by definition \eqref{eq:def_of_offstar} of the flow $\off^*$, the fact that $(\off^t,\oss^t,\ovnu^t)$ is $3\hgamma$-centered -- cf. \eqref{eq:centrality_increase} -- and Fact \ref{fa:central_vs_max_min}, we have that
\begin{eqnarray}
\energy{\trr^t}{\off^*} &=& \sum_e \frac{\os_e^t}{\of'_e}\left(\frac{\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t}\of^t_e\right)^2 \leq \sum_e \frac{\onu_e^t\ohmu_e^t}{\of'_e}\frac{(\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t))^2\of_e^t}{(1-3\hgamma)\ohmu_e^t \hmu(\off^t,\oss^t,\ovnu^t)}\notag\\
&\leq & \frac{1}{(1-3\hgamma)}\sum_e \onu_e^t \frac{(\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t))^2\of_e^t}{\hmu(\off^t,\oss^t,\ovnu^t)\of_e'} = \frac{1}{(1-3\hgamma)}\sum_e \onu_e^t \frac{(\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t))^2\ohmu_e^t}{\hmu(\off^t,\oss^t,\ovnu^t)^2}\notag\\
&\leq & \frac{(1+3\hgamma)}{(1-3\hgamma)}\sum_e \onu_e^t \frac{(\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t))^2}{\hmu(\off^t,\oss^t,\ovnu^t)} =  \frac{(1+3\hgamma)}{(1-3\hgamma)} \frac{\norm{\ohvmu^t-\hmu(\off^t,\oss^t,\ovnu^t)\onev}{\ovnu^t,2}^2}{\hmu(\off^t,\oss^t,\ovnu^t)} \label{eq:energy_estimate_final} \\
& \leq  & \frac{(1+3\hgamma)}{(1-3\hgamma)} 9 \hgamma^2 \hmu(\off^t,\oss^t,\ovnu^t) \leq 10 \hgamma^2 \hmu(\off^t,\oss^t,\ovnu^t)\leq 20 \hgamma^2 \hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1}),\notag
\end{eqnarray}
where we also used the definition \eqref{eq:offprime_def} of the flow $\off'$.


In the light of the above discussion, we can conclude that 
\begin{eqnarray*}
\norm{\hvmu^{t+1}-\hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1})\onev}{\vnu^{t+1},2}^2 &\leq & \sum_e \onu_e^t \left(\frac{\os_e^t}{\onu^t_e\of_e'} (\tf_e^t)^2\right)^2 \leq \left(\sum_{e} \frac{\os_e^t}{\of_e'} (\tf_e^t)^2\right)^2\\
&\leq &  \left(20 \hgamma^2 \hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1})\right)^2 \leq \hgamma^2 \hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1})^2,
\end{eqnarray*}
as $\hgamma\leq \frac{1}{20}$. So, indeed $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ is $\hgamma$-centered. 

Now, to prove that $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ is also $\vsigma$-feasible, we just need to show that for any arc $e$, 
\[
\rho(\tff^t,\off')_e=\frac{|\tf^t_e|}{\of'_e}\leq \frac{1}{2}.
\]
To this end, note that by \eqref{eq:perfect_centering_of_intermediate} and \eqref{eq:energy_estimate_final} we have
\begin{equation}
\label{eq:interior_bound_1}
\hmu(\off^t,\oss^t,\ovnu^t)\rho(\tff^t,\off')_e^2 = \frac{\os_e^t\of'_e}{(\of'_e)^2}(\tf_e^t)^2 = \frac{\os_e^t}{\of'_e}(\tf_e^t)^2\leq \energy{\trr^t}{\tff^t}\leq  \energy{\trr^t}{\off^*} \leq 10 \hgamma^2 \hmu(\off^t,\oss^t,\ovnu^t)\leq \frac{1}{1600} \hmu(\off^t,\oss^t,\ovnu^t).
\end{equation}

Thus, indeed, we can conclude that we obtained a $\hgamma$-centered $\vsigma$-feasible solution $(\ff^{t+1},\ss^{t+1},\vnu^{t+1})$ with $\hmu(\ff^{t+1},\ss^{t+1},\vnu^{t+1})\leq (1-\delta^t)\hmu(\ff^{t},\ss^{t},\vnu^{t})$, as desired.

Now, to prove the second part of the theorem, note first that indeed $\vnu^{t+1}=\ovnu^{t}=\vnu^t$. Next, we can check that the cumulative changes of the vectors $\ff^{t}$ and $\ss^t$ are equal to
\begin{eqnarray*}
f_e^{t+1} &=& (1-\delta^t)\left(1+\frac{\delta^t\hf^t_e}{(1-\delta^t)f_e^t}\right)\left(1-\frac{\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t}\right)\left(1+\frac{\tf^t_e}{\of_e'}\right)f_e^t\\
s_e^{t+1} &=& \left(1-\frac{\delta^t\hf^t_e}{(1-\delta^t)f_e^t}\right)\left(1-\frac{\tf^t_e}{\of_e'}\right)s_e^t,
\end{eqnarray*}
for each arc $e$ in $\hG$. 

As a result, by \eqref{eq:hf_resistances}, we have that for each arc $e$,
\[
(1-\delta^t)r_e^{t+1} = \frac{(1-\delta^t) s_e^{t+1}}{f_e^{t+1}} = \frac{\left(1-\frac{\delta^t\hf^t_e}{(1-\delta^t)f_e^t}\right)\left(1-\frac{\tf^t_e}{\of_e'}\right)s_e^t}{\left(1+\frac{\delta^t\hf^t_e}{(1-\delta^t)f_e^t}\right)\left(1-\frac{\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t}\right)\left(1+\frac{\tf^t_e}{\of_e'}\right)f_e^t}.
\]

Recall that from the discussion above we already know that, for each arc $e$,  $|\frac{\delta^t\hf^t_e}{(1-\delta^t)f_e^t}|=\frac{\delta^t\rho(\hff^t,\ff^t)_e}{(1-\delta^t)}\leq 2\sqrt{\hgamma}\leq \frac{1}{10}$ (cf. \eqref{eq:interior_bound_2}), $|\frac{\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t}|\leq \frac{\hgamma}{(1-\hgamma)} \leq \frac{1}{40}$ (cf. Fact \ref{fa:central_vs_max_min}), and $|\frac{\tf^t_e}{\of_e'}|=\rho(\tff^t,\off')_e\leq \frac{1}{40}$ (cf. \eqref{eq:interior_bound_1}). So, as $r_e^t=\frac{s_e^t}{f_e^t}$, we have that 
\[
(1+\kappa_e^t)=\frac{\left(1-\frac{\delta^t\hf^t_e}{(1-\delta^t)f_e^t}\right)\left(1-\frac{\tf^t_e}{\of_e'}\right)}{\left(1+\frac{\delta^t\hf^t_e}{(1-\delta^t)f_e^t}\right)\left(1-\frac{\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)}{\ohmu_e^t}\right)\left(1+\frac{\tf^t_e}{\of_e'}\right)}
\]
and by performing a simple Taylor expansion approximation we can obtain that 
\[
|\kappa_e^t|\leq 2\left(\frac{\delta^t\rho(\hff^t,\ff^t)_e}{(1-\delta^t)}+ \frac{|\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)|}{\ohmu_e^t}+\rho(\tff^t,\off')_e\right)\leq 4\left(\delta^t\rho(\hff^t,\ff^t)_e+\hkappa_e^t\right),
\]
for each arc $e$, where $\hkappa_e^t:=\frac{|\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t)|}{\ohmu_e^t}+\rho(\tff^t,\off')_e$. 

Clearly, this means, in particular, that $\inorm{\kappa_e^t}\leq 2(\frac{2}{10}+\frac{1}{40}+\frac{1}{40})=\frac{1}{2}$, as desired. So, we just need to show that $\norm{\hvkappa^t}{\vnu^t,2}\leq \frac{1}{16}$ too. To this end, observe that
\begin{eqnarray*}
\norm{\hvkappa^t}{\vnu^t,2}^2 &\leq& 2 \sum_{e} \nu_e^t \left(\frac{(\ohmu_e^t-\hmu(\off^t,\oss^t,\ovnu^t))^2}{(\ohmu_e^t)^2} + \rho(\tff^t,\off')_e^2\right) \\
&\leq& 2\left( \frac{\norm{\ohvmu^t-\hmu(\off^t,\oss^t,\ovnu^t)\onev}{\ovnu^t,2}^2}{(1-\hgamma)^2\hmu(\off^t,\oss^t,\ovnu^t)^2} + \frac{1}{\hmu(\off^t,\oss^t,\ovnu^t)} \sum_e \hmu(\off^t,\oss^t,\ovnu^t) \rho(\tff^t,\off')_e^2\right)\\
&\leq & 2 \left(9 \hgamma^2 + \frac{\energy{\trr^t}{\tff^t}}{\hmu(\off^t,\oss^t,\ovnu^t)} \right) \leq \frac{1}{256},
\end{eqnarray*}
as desired, where we used a combination of Fact \ref{fa:central_vs_max_min}, the fact that $(\off^t,\oss^t,\ovnu^t)$ is $3\hgamma$-centered, as well as, equations \eqref{eq:perfect_centering_of_intermediate} and  \eqref{eq:energy_estimate_final}.
This concludes the proof of the theorem.
